GAPS: Geometry-Aware, Physics-Based, Self-Supervised Neural Garment Draping

Recent neural, physics-based modeling of garment deformations allows faster and visually aesthetic results as opposed to the existing methods. Material-specific parameters are used by the formulation to control the garment inextensibility. This delivers unrealistic results with physically implausible stretching. Oftentimes, the draped garment is pushed inside the body which is either corrected by an expensive post-processing, thus adding to further inconsistent stretching; or by deploying a separate training regime for each body type, restricting its scalability. Additionally, the flawed skinning process deployed by existing methods produces incorrect results on loose garments. In this paper, we introduce a geometrical constraint to the existing formulation that is collision-aware and imposes garment inextensibility wherever possible. Thus, we obtain realistic results where draped clothes stretch only while covering bigger body regions. Furthermore, we propose a geometry-aware garment skinning method by defining a body-garment closeness measure which works for all garment types, especially the loose ones.

==> defs.tex <==
\newif\ifdraft
\draftfalse
\drafttrue

% Comments
\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{magenta}{rgb}{1,0,1}
\definecolor{cyan}{rgb}{0,0.8,0.8}
\definecolor{green}{rgb}{0,0.8,0}
\definecolor{yellow}{rgb}{0.8,0.7,0.1}

\newcommand{\wideemptyfigure}[3]{\begin{figure*}\begin{center}\vspace{#2}\end{center}\caption{#1}\label{#3}\end{figure*}}

\newcommand{\emptyfigure}[3]{\begin{figure}\begin{center}\vspace{#2}\end{center}\caption{#1}\label{#3}\end{figure}}

\ifdraft
 \newcommand{\RC}[1]{{\color{blue}{\bf RC: #1}}}
 \newcommand{\rc}[1]{{\color{blue}{#1}}}
 \newcommand{\SP}[1]{{\color{red}{\bf SP: #1}}}
 \newcommand{\sp}[1]{{\color{red} #1}}
 
 
\else
 \newcommand{\JB}[1]{}
 \newcommand{\jb}[1]{ #1 }
 \newcommand{\NA}[1]{}
 \newcommand{\na}[1]{ #1 }
 \newcommand{\VK}[1]{}
 \newcommand{\vk}[1]{ #1 }
 \newcommand{\SC}[1]{}
 \newcommand{\sc}[1]{ #1 }
 \newcommand{\PF}[1]{}
 \newcommand{\pf}[1]{ #1 }
 \newcommand{\MS}[1]{}
 \newcommand{\ms}[1]{ #1 }
\fi

\newcommand{\comment}[1]{}
\newcommand{\parag}[1]{\vspace{-3mm}\paragraph{#1}}

% Math
\newcommand{\natur}{\mathbb{N}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

% Formalization
\newcommand{\wpatch}{\mathbf{w}_{k}}
\newcommand{\fpatch}{f_{\wpatch}}
\newcommand{\uvdom}{\Omega}
\newcommand{\latrep}{\mathbf{z}}
\newcommand{\latdim}{Z}
% \newcommand{\dfu}{\mathbf{f}_{\latrep k_{u}}}
% \newcommand{\dfv}{\mathbf{f}_{\latrep k_{v}}}
\newcommand{\dfu}{\mathbf{f}^{(k)}_{\latrep_{u}}}
\newcommand{\dfv}{\mathbf{f}^{(k)}_{\latrep_{v}}}
\newcommand{\ptuv}{\mathbf{q}}
\newcommand{\ptthreed}{\mathbf{p}}
\newcommand{\metric}{g_{k}}
% \newcommand{\jac}{\mathbf{J}_{\latrep k_{\ptuv}}}
\newcommand{\jac}{\mathbf{J}^{(k)}_{\latrep_{\ptuv}}}
\newcommand{\shapecol}{\mathcal{C}}
\newcommand{\shapeA}{S_{i}}
\newcommand{\shapeB}{S_{j}}
\newcommand{\metricA}{\metric^{(\shapeA)}}
\newcommand{\metricB}{\metric^{(\shapeB)}}
\newcommand{\latrepA}{\latrep_{i}}
\newcommand{\latrepB}{\latrep_{j}}
\newcommand{\latrepAB}{\latrep_{ij}}
\newcommand{\norm}[2]{\left\lVert#1\right\rVert_{#2}^{2}}
\newcommand{\frobnormsq}[1]{\norm{#1}{\text{F}}}
\newcommand{\ltwonormsq}[1]{\norm{#1}{2}}
% \newcommand{\frobnormsq}[1]{\left\lVert#1\right\rVert_{\text{F}}^{2}}
% \newcommand{\ltwonormsq}[1]{\left\lVert#1\right\rVert_{\text{2}}^{2}}
\newcommand{\metricdiff}{\mathcal{D}_{s}}
\newcommand{\expected}[1]{\mathop{{}\mathbb{E}}_{#1}}
\newcommand{\shapecolsize}{C}
\newcommand{\metricchange}{\mathcal{D}_{l}}
\newcommand{\metricinterp}{\mathcal{D}_{ip}}
\newcommand{\interpparam}{\alpha}
\newcommand{\patchidx}{k}
\newcommand{\numpatches}{K}
\newcommand{\sumpatches}{\sum_{\patchidx = 1}^{\numpatches}}
\newcommand{\surfspeed}{\mathcal{D}_{sp}}

% Losses
\newcommand{\lossmetcon}{\mathcal{L_{\text{mc}}}}
\newcommand{\lossinterp}{\mathcal{L_{\text{ip}}}}
\newcommand{\lossspeed}{\mathcal{L}_{sp}}
\newcommand{\losscd}{\mathcal{L}_{CD}}
\newcommand{\lossfinal}{\mathcal{L}}
\newcommand{\wmetcon}{\alpha_{\text{mc}}}
\newcommand{\winterp}{\alpha_{\text{ip}}}
\newcommand{\wspeed}{\alpha_{\text{sp}}}

% Models.
\newcommand{\ours}{OUR}
\newcommand{\oursad}{OURS-AD}
\newcommand{\atlasnet}{AN}
\newcommand{\dsr}{DSR}
\newcommand{\cyccon}{CC}
\newcommand{\nricp}{nrICP}

% Evaluation metrics
\newcommand{\mdist}{m_{sL2}}
\newcommand{\mrank}{m_{r}}
\newcommand{\mpckauc}{m_{\text{AUC}}}

\newcommand{\crefrangeconjunction}{--}
\def\poincare/{Poincar\'e}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}
%%replaces missing figs
%\makeatletter
%\def\Ginclude@graphics#1{%
%    \parpic(\Gin@@ewidth,\Gin@@eheight)[d]{#1}\picskip{0}}%
%\makeatother
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}
%yaron added these
\def\eg{\textit{e.g.}}
\def\etal{\textit{et al.}~}
\def\etc{\textit{etc.}~}
\def\ie{\textit{i.e.}}
% MATH -----------------------------------------------------------
\newcommand{\nrm}[1]{\left\Vert#1\right\Vert}
\newcommand{\cut}{\bar}
\newcommand{\Norm}[1]{\lvert \! \lvert \! \lvert #1 \rvert \! \rvert \! \rvert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\babs}[1]{\Big \vert#1 \Big \vert}
\newcommand{\tr}[1]{\mathrm{tr} #1}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\parr}[1]{\left (#1\right )}
\newcommand{\brac}[1]{\left [#1\right ]}
\newcommand{\ip}[1]{\left \langle #1 \right \rangle }
\newcommand{\Real}{\mathbb R}
\newcommand{\Natural}{\mathbb N}
\newcommand{\grad}{\nabla}
\newcommand{\leftcut}{\triangleleft}
\newcommand{\rightcut}{\triangleright}
\newcommand{\ingrad}{\mathrm{grad}}
\newcommand{\p}[1]{\bar#1}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\too}{\rightarrow}
\newcommand{\BX}{\mathbf{B}(X)}
%\newcommand{\A}{\mathcal{A}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\bbar}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}} %wide tilde
\newcommand{\wh}[1]{\widehat{#1}} %wide hat
\newcommand{\eop}{\hfill $\Box$}
\newcommand{\area}[1]{\abs{#1}}


\def\mobius/{M{\"o}bius}
\newcommand {\closure}[1]{\textrm{Closure}(#1)} %closure of a set
\newcommand {\interior}[1]{\textrm{Interior}(#1)} %interior of a set
\newcommand {\1}{\mathrm{\textbf{1}}}
\newcommand {\re}{\mathrm{Re}\,}
\newcommand {\im}{\mathrm{Im}\,}
\newcommand {\ii}{\mathrm{{i}}}
\def \diag{\mathrm{diag}}
\newcommand{\cg}[1]{{\textcolor{red}{#1}}}
\newcommand{\fnorm}[1]{\norm{#1}_F}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\polyc}[1]{\brac{#1}} %polygonal curve
\newcommand{\cpolyc}[1]{\brac{#1}^\circ} %closed polygonal curve
%\newcommand{\length}[1]{\mathrm{length}(#1)}
\def \length{\mathrm{length}}
% Yaron added -----------------------------------------------------------------
\def \AA{\mathcal{A}} %for affine map
\def \EE{\mathcal{E}} %for affine map
\def \P{\mathcal{P}} %landmarks on A
\def \Q{\mathcal{Q}} %landmarks on B
\def \II{\mathcal{I}} %index set
% Special notations -----------------------------------------------------------
\def \MM{{\mathcal{M}}} %the smooth surface M
\def \NN{{\mathcal{N}}} %neighbors
\def \SS{{\mathcal{S}}} %the smooth surface S
\def \graph{\mathcal{G}} %the cut tree
\def \pairs{\mathcal{P}} %the cut tree
%\def \VV{\mathcal{V}} %vertices of the cut-graph
%\def \EE{\mathcal{E}} %edges of the graph cut
%\def \sptree{\mathcal{T}}
\def \f{f} %the bijection
\def \m{\mathrm{m}} %mobius transformation
\def \d{\mathrm{d}}
\def \A{\mathrm{\textbf{A}}} % triangular mesh
\def \B{\mathrm{\textbf{B}}} % triangular mesh
\def \Acut{\bar{\mathrm{\textbf{A}}}} % triangular mesh
\def \Bcut{\bar{\mathrm{\textbf{B}}}} % triangular mesh
\newcommand \seamA{\alpha}
\newcommand \seamB{\beta}
\newcommand \seamAl{\seamA^l}
\newcommand \seamAr{\seamA^r}
\newcommand \seamBl{\seamB^l}
\newcommand \seamBr{\seamB^r}
\newcommand \hyp{\mathbb{H}^2}
\def \Mc{\mathrm{\textbf{M}^\circ}} % mesh / surface
\def \Mo{\textbf{M}} % cut mesh / surface
\def \M{\mathrm{\textbf{M}}}

\def\Vc{\V}
\def\Vo{\barb{\V}}
\def\embc{\Psi}
\def\embo{{\bbar{\Psi}}}


\def \covPhi{\wh{\Psi}} %the mapping of the tiled M
\def \covM{\wh{\textbf{M}}} %tiled M
\def \F{\mathrm{\textbf{T}}} % face set
\def \E{\mathrm{\textbf{E}}} % edge set
\def \V{\mathrm{\textbf{V}}} % vertices set
\def \W{\mathrm{\textbf{W}}} % subset of vertices
\def \sphere{\mathbb{S}} %sphere
\def \vecx{\mathrm{\textbf{x}}} % vector in \Real^3
\def \vecX{\mathrm{\textbf{X}}} % collection of vectors in \Real^3
\def \vecy{\mathrm{\textbf{y}}} % vector in \Real^3
\def \vecY{\mathrm{\textbf{Y}}} % collection of vectors in \Real^3
\def \vecz{\mathrm{\textbf{z}}} % vector in \Real^3
\def \vecv{\mathrm{\textbf{v}}} % vector in \Real^3
\def \vecu{\mathrm{\textbf{u}}} % vector in \Real^3
\def \vece{\mathrm{\textbf{e}}} % the standard vector basis in  \Real^3
\def \vecp{\mathrm{\textbf{p}}} % vector in \Real^3
\def \vecq{\mathrm{\textbf{q}}} % vector in \Real^3
\def \vecc{\mathrm{\textbf{c}}} % vector of conformal factors
\def \vecdel{\mbox{\boldmath$\delta$}} %the translation vector delta
\def \veceta{\mbox{$\eta$}} %the translation vector eta
\def \vecgam{\mbox{\boldmath$\gamma$}} %the translation vector gamma
\def \vecsig{\mbox{\boldmath$\sigma$}} %the translation vector delta
\def \vecmu{\mbox{\boldmath$\mu$}} %the translation vector delta
\def \v{\mbox{\boldmath$v$}} %the vertices
\def \w{\mbox{\boldmath$w$}} %the image vertices
\def \dist{ \mathrm{dist} }
\def \Dist{ \mathrm{Dist} } %the Lipschitz distance
\def \dil{ \mathrm{dil} } %the symmetry dilation of a map
\def \ang{ \mathrm{Angle}} %the rotation angle of a matrix
\def \onering{ \mathcal{R} }
\def \FC{\mathcal{F}_{C}} %the C-Lipschiz maps
\def \FF{\mathcal{F}} %bijective maps
\def \OOmega{\mbox{\boldmath$\Omega$}} %planar domain
\def \C{\mathcal{C}} %the convex space of bounded from below the signed sv.
%\def \etal{et al.,~}


